StreetNav: Leveraging Street Cameras to Support Precise Outdoor Navigation for Blind Pedestrians

Blind and low-vision (BLV) people rely on GPS-based systems for outdoor navigation. GPS's inaccuracy, however, causes them to veer off track, run into obstacles, and struggle to reach precise destinations. While prior work has made precise navigation possible indoors via hardware installations, enabling this outdoors remains a challenge. Interestingly, many outdoor environments are already instrumented with hardware such as street cameras. In this work, we explore the idea of repurposing existing street cameras for outdoor navigation. Our community-driven approach considers both technical and sociotechnical concerns through engagements with various stakeholders: BLV users, residents, business owners, and Community Board leadership. The resulting system, StreetNav, processes a camera's video feed using computer vision and gives BLV pedestrians real-time navigation assistance. Our evaluations show that StreetNav guides users more precisely than GPS, but its technical performance is sensitive to environmental occlusions and distance from the camera. We discuss future implications for deploying such systems at scale.

==> sec04-system.tex <==
% In this section, we introduce a navigation system that we are currently developing to answer RQ2: \textit{How should street camera-based systems be designed to address the challenging aspects of outdoor navigation?} The system consists of three components: \textit{(i)} street camera, \textit{(ii}) computational server,  and \textit{(iii)} smartphone app. These components interact with each other to facilitate two navigation modes that together address BLV people's challenges to outdoor navigation, which we discovered in our formative interviews. 


% \subsection{System Components}

% % The system consists of three main components: (i) street camera, (ii) video processing pipeline, and (iii) smartphone application.

% \subsubsection*{\textbf{Street camera}}
% The system uses a street-level view camera which is part of the NSF PAWR COSMOS wireless edge-cloud testbed in NYC~\cite{raychaudhuri2020challenge,yang2020cosmos}. The camera is mounted at the second floor of the Columbia Mudd building, viewing a four-way street intersection at 120$^\textrm{th}$ St.\ and Amsterdam Ave., NYC, as shown in Figure~\ref{fig:camera_location_view}. Anonymized video samples (without special gestures) from COSMOS cameras, including the one used in this study, can be found in~\cite{cosmos-cameras}. The \textit{real-time} video feed from the camera is directly streamed onto one of COSMOS' computational servers for processing~\cite{ghasemi2023real,ghasemi2023video}.
% \begin{figure}
% \centering
% \includegraphics[width=0.98\linewidth]{images/ceal-camera.pdf}
% \caption{The COSMOS camera deployed at the 2\textsuperscript{nd} floor of Columbia's Mudd building and its view of 120$^\textrm{th}$ St.\ and Amsterdam Ave.\ intersection, NYC.~\cite{cosmos-cameras, yang2020cosmos}}
% \label{fig:camera_location_view}
% \end{figure}

\sloppy
{
\subsubsection*{\textbf{Video processing pipeline}}
% A video processing pipeline is deployed on one of the COSMOS testbed's edge servers. The server runs Ubuntu 20.04 with an Intel Xeon CPU@2.60GHz and an NVIDIA V100 GPU. 

% \textit{Object detection and tracking.} This pipeline decodes and processes the \textit{real-time} video feed from the camera and is developed using GStreamer~\cite{taymans2013gstreamer}, a framework for building optimized video analytics applications. It is equipped with the state-of-the-art YOLOv8 model~\cite{terven2023comprehensive} as an object detector and the Nvidia DCF-based tracker to track pedestrians and vehicles. This tracker assigns a unique identification number (ID) to each detected object during tracking. 
\textcolor{blue}{[todo] adding the evaluation results for tracking} 

% \textit{Pedestrian signal detection.} Moreover, the pipeline uses \textcolor{blue}{X method/model [todo]} to identify pedestrian signals. 

% \textit{Perspective transformation.} To transform pixel coordinates from a specific camera view to a top-down view of the intersection, we designed a feed-forward neural network that we call \textit{CoordinateTransformNet}. The primary goal of \textit{CoordinateTransformNet} is to provide a mapping from the input coordinates in the camera's view to the corresponding points in the top view, leveraging the training dataset derived from manually annotated correspondences. The transformation of coordinates from one perspective to another is fundamentally a regression problem \textcolor{blue}{([todo-Mahshid] add reference)} where the network has to learn a mapping from input coordinates to output coordinates. Therefore, CoordinateTransformNet's architecture consists of:
% \begin{itemize}
%     \item \textbf{Input layer:} Accepts 2D pixel coordinates $(x, y)$.
%     \item \textbf{Intermediate layers:}
%     \begin{itemize}
%         \item 64 neurons with ReLU activation.
%         \item 128 neurons with ReLU activation.
%         \item 64 neurons with ReLU activation.
%     \end{itemize}
%     \item \textbf{Output layer:} Produces transformed 2D coordinates.
% \end{itemize}
% Using the camera view and the corresponding top view of the same intersection, obtained by \textit{CoordinateTransformNet}, the system finds visual correspondences to generate a bird's-eye view representation of the environment (Figure~\ref{fig:teaser}d).
}

% \textit{Traffic light status detection.} \textcolor{blue}{[todo]-----------------------------------------------------------------------------------------------------------------------------------------}

% \textit{Navigation map.\textcolor{blue}{[not sure about the title]}} Additionally, it stores the map information that includes labeled regions (e.g., streets, crosswalks, sidewalks, pedestrian lights) and the location of relevant POIs (e.g., pharmacy, café) within the bird's-eye view representation. Similar to prior work in indoor navigation~\cite{ahmetovic_navcog_2016, sato_navcog3_2019, guerreiro_cabot_2019}, the map information is prepared manually by an administrator and loaded onto the server beforehand.
% The computational server is physically located within the same building onto which the cameras are mounted to reduce latency.


% \subsubsection*{\textbf{Smartphone application}}
% Figure~\ref{fig:teaser}a--b shows the iOS app that acts as an interface between the user and the computational server, enabling them to access the map information and to receive real-time audio feedback via a Bluetooth earpiece. 
% To alleviate concerns around revealing private identifiable information from the video feeds (e.g., pedestrian's faces and vehicle's license plate), the server only sends processed information such as navigation instructions, positions and generic labels of obstacles (e.g., ``vehicle'' at 2 o'clock) to the smartphone app instead of the video itself.  

% does not share the video feed with the smartphone app. Instead, processed outputs such as their positions on the bird's-eye view and generic labels (e.g., ``vehicle'' and ``pedestrian'') are sent over.

% \subsection{Our Testbed}

% What constitutes our system. Where is it. 2 cameras a four-way street intersection. One is at 2nd floor and the other is at 12th floor. All computation happens on the server that is connected directly to the cameras. Nothing happens on the app itself. The app is just meant for interfacing with the camera system.





% \subsection{User Interaction}
% BLV pedestrians use the smartphone app to establish a connection with the server via a localization mechanism. Once localized, users are offered two navigation modes: (i) guidance mode, and (ii) exploration mode. 



% \subsubsection*{\textbf{Pedestrian Localization}} 
% To determine the user's position on the bird's-eye view map, the system must differentiate them from other pedestrians on the street. We achieved this by introducing an action recognition module that can identify users from the second floor camera feed. The smartphone app asks the user to initialize the system with their current position by simply waving one hand above their head for a few seconds, which is detected by the action recognition module. We chose this action based on discussions with several BLV individuals and most agreed that this single-handed action was both convenient and socially acceptable to them. Internally, the action recognition module is implemented as a CLIP model~\cite{radford_learning_2021} that computes visual similarity of each detected pedestrian from the second floor camera with the following language prompts: ``\textit{person walking}'' and ``\textit{person waving hand}.'' We experimentally fine-tuned the confidence thresholds.
% To reduce false positives, we perform localization exactly at the time when user attempts to establish a connection.


\subsubsection*{\textbf{Navigation modes}}
To address the challenging aspects of outdoor navigation that we identified from our formative study, we designed the street camera-based navigation system to support the following two modes of navigation:

% \textit{(i) Guidance Mode}. Figure~\ref{fig:teaser}a shows this mode, where BLV users can choose a destination from the list of nearby POIs and receive real-time audio feedback in the form of turn-by-turn instructions. Similar to prior work in indoor navigation~\cite{ahmetovic_navcog_2016}, we represent the birds-eye view map as a graph representation consisting of POIs and street corners as nodes that act as way-points. The knowledge of the user's precise position enables the system to provide audio cues that help prevent veering off the path between way-points (Section~\ref{sec:challenge-1}).






To address BLV users' challenges to avoid obstacles while following instructions (Section~\ref{sec:challenge-2}), the street camera-based system notifies users of obstacles ---both moving and fixed--- by specifying their relative spatial location and category (e.g., by announcing ``\textit{pedestrian at 2'o clock, 5 feet away}''). Our current implementation offers support for dynamic obstacles such as pedestrians and vehicles, along with fixed ones such as poles, trashcans, and parked vehicles. Internally, we implement this by tracking all these elements within the space and predicting positional overlaps in bird's-eye view. For dynamic obstacles, specifically vehicles, we plan on adapting our prediction module to also account for their speed. 

% To address BLV people’s challenges in crossing street intersections safely (Section~\ref{sec:challenge-3}), the system dynamically updates the internal graph representation to temporarily remove crosswalks that have pedestrian signals reading ``wait’' and reinstates it when they read: ``walk.‘’ Once the system reinstates the crosswalk, it provides users precise information about the time remaining to cross and the distance to the other end of the crosswalk. The system gathers this information by first automatically detecting the signal state (i.e., walk vs. wait) and then computing the time it takes to change over a complete cycle. 


% \textit{ (ii) Exploration Mode}. Figure~\ref{fig:teaser}b shows this mode, where BLV users can choose to navigate the environment without any specific destination in mind. Similar to guidance mode, this mode also provides users real-time feedback to prevent veering (Section~\ref{sec:challenge-1}), avoid obstacles (Section~\ref{sec:challenge-2}), and cross street intersections safely (Section~\ref{sec:challenge-3}). Additionally, this mode is designed to address BLV users' challenge to anticipate environment layouts (Section~\ref{sec:challenge-1}). The user can scrub their finger on the smartpho
ne to learn (via haptic feedback) the bird's-eye view map's shape and layout, which has been found to provide BLV people spatial understanding of the environment~\cite{jain_i_2023}. Prior work on image accessibility also shows that direct manipulation via touchscreen-based interfaces helps BLV 
% users effectively explore images~\cite{lee_imageexplorer_2022}. Our current implementation allows users to move their finger across the map on the smartphone app, reading out the corresponding region labels (e.g., street, crosswalk, sidewalk). We plan on extending this touchscreen-based exploration tool to also convey users' current position and POIs.














% \section{Technical Details / Back-end System}

% \subsection{Localization}

% \subsection{Internal Graph Structure - turn by turn nav}

% \subsection{Obstacle Awareness}

% \subsection{Street Crossing}


% \subsection{Veering }


==> sec05-future_work.tex <==
In addition to extensions mentioned earlier, we are developing our system's audio cues for rendering real-time feedback in the two navigation modes. We plan on conducting pilot studies to identify and fix any technical issues and to iterate over the system's design. To evaluate the street camera-based navigation system (i.e., to answer RQ3) we will conduct user studies with BLV pedestrians. In this study, we will compare participants' experience of navigating street intersections using the proposed system and the GPS apps. In addition to directly asking participants to share their overall impressions, we plan to analyze participants’ behaviors and system usage logs. Our aim is to understand the extent to which street cameras can be used to support precise and real-time outdoor navigation.
% Our aim is to gather
% insights from this study that can assist game developers in designing similar tools for their own games, enabling BLV
% players to experience a sense of fun within 3D game environments that is on par with what sighted players enjoy


% We want to also evaluate BLV people's attitude towards security and privacy aspects of the system that records and uses public information.

==> sec07-social_factors.tex <==
\label{sec:social_factors}

\revision{
StreetNav’s user evaluations on our testbed shows its promise in increasing BLV pedestrians’ independence and safety during outdoor navigation. StreetNav’s widespread adoption beyond this testbed, however, may be influenced by several social factors. For example, government and legal authorities may need to adapt public policy to support accommodations that enable access to the street camera video feed, bystanders may raise privacy and security concerns with the use of these cameras, and BLV users themselves may not feel comfortable interacting with StreetNav in public. It is important that StreetNav’s current design evolves to consider such social factors, before it is deployed at scale.
}


\revision{
To identify these social factors, we performed a series of semi-structured interviews with different stakeholders that may affect, or be affected by, StreetNav’s widespread adoption. Specifically, we aim to identify the social factors around policy for accessing street cameras, privacy and security concerns with its use, social acceptability and trust in the technology, and concerns around long-term use and adoption of such technology. Thus, we interviewed representatives from four major stakeholder categories, \textbf{(1) government authorities}: leadership from department of transportation to discuss policy implications; \textbf{(2) general public}: bystanders and local shop owners/staff to discuss privacy, security, and social acceptability concerns; \textbf{(3) primary users}: BLV pedestrians to discuss similar concerns as well as trust in the technology, and \textbf{(4) advocacy groups:} leadership from blind-serving organization to discuss concerns around technology adoption and policy implications.
}


\subsubsection*{\textbf{Participants}}
\revision{}


\subsubsection*{\textbf{Procedure}}
\revision{}


\subsubsection*{\textbf{Data Analysis}}
\revision{}
